Towards Fairness of Cryptocurrency Payments

Motivated by the great success and adoption of Bitcoin, a number of cryptocurrencies such as Litecoin, Dogecoin, and Ethereum are becoming increasingly popular. Although existing blockchain-based cryptocurrency schemes can ensure reasonable security for transactions, they do not consider any notion of fairness. Fair exchange allows two players to exchange digital "items", such as digital signatures, over insecure networks fairly, so that either each player gets the other's item, or neither player does. Given that blockchain participants typically do not trust each other, enabling fairness in existing cryptocurrencies is an essential but insufficiently explored problem. In this paper, we explore the solution space for enabling the fair exchange of a cryptocurrency payment for a receipt. We identify the timeliness of an exchange as an important property especially when one of the parties involved in the exchange is resource-constrained. We introduce the notion of strong timeliness for a fair exchange protocol and propose two fair payment-for-receipt protocol instantiations that leverage functionality of the blockchain to achieve strong timeliness. We implement both and compare their security and efficiency.

==> chapters/acknowledgment.tex <==
%!TEX root = ../submission.tex
\ifsubmission
\else
\section*{Acknowledgments}
This work was supported in part by the Academy of Finland project
``Cloud Security Services'' (283135).
\fi
\label{sec:ack}




==> chapters/background.tex <==
%!TEX root = ../submission.tex
\section{Background}
\label{sec:background}





==> chapters/conclusion.tex <==
%!TEX root = ../submission.tex
\section{Conclusion and Future Work}
\label{sec:conclusion}



==> chapters/design_overview.tex <==
%!TEX root = ../submission.tex
\section{The Carousel approach}
\label{sec:carouselApproach}



==> chapters/extensions.tex <==
%!TEX root = ../submission.tex
\section{Variations and Extensions}
\label{sec:extensions}



==> chapters/fair_exchange4.tex <==
%!TEX root = ../submission.tex
\subsection{Non-Invasiveness and Strong fairness}
\label{witness}
%\ghassan{IMHO, this fits better as a subsection of this section}

%Jager~\cite{Jager2015} constructs a {\em time-lock encryption} scheme, where a sender is able to encrypt a ciphertext, such that not even a computationally powerful (but reasonably bounded) adversary is able to learn any non-trivial information about the message before the deadline. Once the deadline has passed, even receivers with relatively limited computational resources are immediately able to decrypt. Decryption is non-interactive, in the sense that there is no communication between the sender and receivers except for the initial, unidirectional transmission of the ciphertext, or among receivers. They define the ``time'' in terms of the \ghassan{length?} length of Bitcoin blockchain.\ghassan{i am a bit confused how does this fit here.}

Our final proposal leverages \emph{witness encryption} to realize fair exchange. In what follows, we start by describing the functionality of the witness encryption schemes %how to achieve time-locked encryption in the blockchain based on witness encryption schemes,
and then show how to construct fair exchanges by leveraging such functionality.

\subsubsection{Witness Encryption}

Witness encryption was first proposed by Garg et al. in~\cite{Garg2013}.
A witness encryption scheme is associated with a specific NP-relation $(x, w) \in R$, where $x$ is a ``statement'' and $w$ is a ``witness''.
It allows the sender to encrypt a message $m$ with respect to statement $x$ as $c \leftarrow Enc_R(x,m)$.
Any receiver who knows the witness $w$ that satisfies $(x,w) \in R$ can decrypt this ciphertext $c$ as $m = Dec_R(c,w)$.
Intuitively, one may think of a statement $x$ as a ``public key'', such that any witness $w$ with $(x, w) \in R$ can be used as a corresponding ``secret key''. A secure witness encryption scheme essentially guarantees that no adversary is able to learn any nontrivial information about the message $m$, unless it already ``knows'' a witness $w$ for $(x, w) \in R$. %Witness encryption schemes with this property are called extractable.


\subsubsection{Our Proposal}\label{subsec:our}
%--------------

We show that the basic protocol in Section~\ref{invasive} can be made non-invasive by leveraging witness encryption. To this end, we assume that each fair payment protocol instance run between $\Alice$ and $\Bob$ has a unique ID. We define an NP-relation $R$ as follows:
\begin{enumerate}
\item The statement $x$ has the form $(T_{\mathsf{abort}_i}, T_{\sigma_i})$, where $T_{\mathsf{abort}_i}$ is a signature by $\Alice$ and $T_{\sigma_i}$ is a signature by $\Bob$ that contains the encryption itself.
\item The blockchain contains $T_{\sigma_i}$ but does not contain $T_{\mathsf{abort}_i}$ \ghassan{what?why? i dont follow}.
\end{enumerate}

In our enhanced proposal, $\Bob$ broadcasts the signature $\sigma_i$ encrypted using a witness encryption with this NP-relation. This ensures that no other entity can decrypt $\sigma_i$ and acquire the signature until it is confirmed in the blockchain. When $\Bob$ wishes to spend $T_{\sigma_i}$, all miners decrypt $Enc_R(x,\sigma_i)$ and check the validity of $\sigma_i$. If $\sigma_i$ is not a valid signature, $\Alice$ is still able to get her money back by making a $T_{\mathsf{abort}_i}$ transaction.

This extension ensures the following properties:

\begin{itemize}
\item {\bf Effectiveness:} If both players behave correctly, $\Bob$ will receive the payment by publishing a $T_{\sigma_i}$ transaction, and $\Alice$ will obtain her desired signature when $T_{\sigma_i}$ is confirmed.
\item {\bf Fairness:} $\Bob$ can only receive the payment when $T_{\sigma_i}$ is confirmed. Similarly, once $T_{\sigma_i}$ is confirmed, $\Alice$ receives her signature.
\item {\bf Timeliness:} The protocol will be terminated after either $T_{\sigma_i}$ or $T_{\mathsf{abort}_i}$ is confirmed. In the former case, the exchange is successfully completed. In the latter case, the exchange is terminated with strong fairness being guaranteed.
%Alice does not get anything about the signature\ghassan{does not get anything-> does not reveal any meaningful information or does not leak any bit or?}.
\item {\bf Non-invasiveness:} $\sigma_i$ is non-invasive since it can correspond to arbitrary signatures %\ghassan{I still think that the notion of arbitrary signatures should be better clarified in the preliminaries}
that $\Alice$ can acquire when the transaction is confirmed. %\ghassan{we need to say what we mean by a normal signature}
\end{itemize}




==> chapters/limitations.tex <==
%!TEX root = ../submission.tex
\section{Security Analysis}
\label{sec:limitations}


==> chapters/related_work.tex <==
%!TEX root = ../submission.tex
\section{Related Work}
\label{sec:related_work}
\ghassan{while i agree to generally include related work towards the end of the paper, i think that in this particular case it might be helpful to put in the preliminaries section and rename that section to ``Preliminaries and Related Work}
Elaine Shi's protocol... only payment to payment.



==> chapters/requirements.tex <==
%!TEX root = ../submission.tex
\section{Requirements} 


